JWST's PEARLS: Mothra, a new kaiju star at z=2.091 extremely magnified by MACS0416, and implications for dark matter models

We report the discovery of Mothra, an extremely magnified monster star, likely a binary system of two supergiant stars, in one of the strongly lensed galaxies behind the galaxy cluster MACS0416. The star is in a galaxy with spectroscopic redshift $z=2.091$ in a portion of the galaxy that is parsecs away from the cluster caustic. The binary star is observed only on the side of the critical curve with negative parity but has been detectable for at least eight years, implying the presence of a small lensing perturber. Microlenses alone cannot explain the earlier observations of this object made with the Hubble Space Telescope. A larger perturber with a mass of at least $10^4$\,\Msun\ offers a more satisfactory explanation. Based on the lack of perturbation on other nearby sources in the same arc, the maximum mass of the perturber is $M< 2.5\times10^6$\,\Msun, making it the smallest substructure constrained by lensing above redshift 0.3. The existence of this millilens is fully consistent with the expectations from the standard cold dark matter model. On the other hand, the existence of such small substructure in a cluster environment has implications for other dark matter models. In particular, warm dark matter models with particle masses below 8.7\,keV are excluded by our observations. Similarly, axion dark matter models are consistent with the observations only if the axion mass is in the range $0.5\times10^{-22}\, {\rm eV} < m_a < 5\times10^{-22}\, {\rm eV}$.

==> Builders_Authors_AA.tex <==
%%% PEARLS Builders.tex %%% Contains all PEARLS builders' affils and ackns
%%% (ordered alphabetically by last name, as discussed in telecon Wed 31 May 2023)
%%% These should be included in all PEARLS papers unless they don't want to
%%%
%%% Author order for PEARLS papers (described by Rogier in telecon Wed 31 May 2023):
%%%		Group 1: small handful of authors who did the bulk of the work a given paper
%%%		Group 2: authors in this file (unless some are moved to Group 1)
%%%		Group 3: other authors who provide input, comments, feedback etc

\author[0000-0001-7410-7669]{Dan Coe} %%% dcoe@stsci.edu
\institute{Space Telescope Science Institute, 3700 San Martin Drive, Baltimore, MD 21218, USA}
\institute{Association of Universities for Research in Astronomy (AURA) for the European Space Agency (ESA), STScI, Baltimore, MD 21218, USA}
\institute{Center for Astrophysical Sciences, Department of Physics and Astronomy, The Johns Hopkins University, 3400 N Charles St. Baltimore, MD 21218, USA}

\author[0000-0003-3329-1337]{Seth H. Cohen} %%% seth.cohen@asu.edu
\institute{School of Earth and Space Exploration, Arizona State University,
Tempe, AZ 85287-1404, USA}

\author[0000-0003-1949-7638]{Christopher J. Conselice} %%% conselice@gmail.com
\institute{Jodrell Bank Centre for Astrophysics, Alan Turing Building,
University of Manchester, Oxford Road, Manchester M13 9PL, UK}

\author[0000-0002-9816-1931]{Jordan C. J. D'Silva} %%% jordan.dsilva@research.uwa.edu.au
\institute{International Centre for Radio Astronomy Research (ICRAR) and the
International Space Centre (ISC), The University of Western Australia, M468,
35 Stirling Highway, Crawley, WA 6009, Australia}
\institute{ARC Centre of Excellence for All Sky Astrophysics in 3 Dimensions
(ASTRO 3D), Australia}

\author[0000-0001-9491-7327]{Simon P. Driver} %%% Simon.Driver@icrar.org
\institute{International Centre for Radio Astronomy Research (ICRAR) and the
International Space Centre (ISC), The University of Western Australia, M468,
35 Stirling Highway, Crawley, WA 6009, Australia}

\author[0000-0003-1625-8009]{Brenda Frye} %%% brendafrye@gmail.com
\institute{Steward Observatory, University of Arizona, 933 N Cherry Ave,
Tucson, AZ, 85721-0009, USA}

\author[0000-0001-9440-8872]{Norman A. Grogin} %%% nagrogin@stsci.edu
\institute{Space Telescope Science Institute,
3700 San Martin Drive, Baltimore, MD 21218, USA}

\author[0000-0003-1268-5230]{Rolf A. Jansen} %%% rolfjansen.work@gmail.com
\institute{School of Earth and Space Exploration, Arizona State University,
Tempe, AZ 85287-1404, USA}

\author[0000-0002-6610-2048]{Anton M. Koekemoer} %%% koekemoer@stsci.edu
\institute{Space Telescope Science Institute,
3700 San Martin Drive, Baltimore, MD 21218, USA}

\author[0000-0001-6434-7845]{Madeline A. Marshall} %%% madeline_marshall@outlook.com
\institute{National Research Council of Canada, Herzberg Astronomy \&
Astrophysics Research Centre, 5071 West Saanich Road, Victoria, BC V9E 2E7,
Canada}
\institute{ARC Centre of Excellence for All Sky Astrophysics in 3 Dimensions
(ASTRO 3D), Australia}

\author[0000-0001-6342-9662]{Mario Nonino} %%% nnn.mario@gmail.com
\institute{INAF-Osservatorio Astronomico di Trieste, Via Bazzoni 2, 34124
Trieste, Italy}

\author[0000-0003-3382-5941]{Nor Pirzkal} %%% npirzkal@stsci.edu
\institute{Space Telescope Science Institute,
3700 San Martin Drive, Baltimore, MD 21218, USA}

\author[0000-0003-0429-3579]{Aaron Robotham} %%% aaron.robotham@uwa.edu.au
\institute{International Centre for Radio Astronomy Research (ICRAR) and the
International Space Centre (ISC), The University of Western Australia, M468,
35 Stirling Highway, Crawley, WA 6009, Australia}

\author[0000-0001-7016-5220]{Michael J. Rutkowski} %%% michael.rutkowski@mnsu.edu
\institute{Minnesota State University-Mankato,  Telescope Science Institute,
TN141, Mankato MN 56001, USA}

\author[0000-0003-0894-1588]{Russell E. Ryan, Jr.} %%% rryan.asu@stsci.edu
\institute{Space Telescope Science Institute,
3700 San Martin Drive, Baltimore, MD 21218, USA}

\author[0000-0002-7265-7920]{Jake Summers} %%% jakesummers7200@gmail.com
\institute{School of Earth and Space Exploration, Arizona State University,
Tempe, AZ 85287-1404, USA}

\author[0000-0001-9052-9837]{Scott Tompkins} %%% satompki@asu.edu
\institute{School of Earth and Space Exploration, Arizona State University,
Tempe, AZ 85287-1404, USA}

\author[0000-0001-9262-9997]{Christopher N. A. Willmer} %%% cnawillmer@gmail.com
\institute{Steward Observatory, University of Arizona,
933 N Cherry Ave, Tucson, AZ, 85721-0009, USA}

\author[0000-0001-8156-6281]{Rogier A. Windhorst}%%% Rogier.Windhorst@gmail.com
\institute{School of Earth and Space Exploration, Arizona State University,
Tempe, AZ 85287-1404, USA}

\author[0000-0001-7592-7714]{Haojing Yan} %%% yanhaojing@gmail.com
\institute{Department of Physics and Astronomy, University of Missouri,
Columbia, MO 65211, USA}



%\sn \software{ Astropy: \url{http://www.astropy.org} \citep{Robitaille2013,Astropy2018};\ IDL Astronomy Library: \url{https://idlastro.gsfc.nasa.gov}
%\citep{Landsman1993};\ Photutils:
%\url{https://photutils.readthedocs.io/en/stable/} \citep{Bradley20};\
%\ProFound: \url{https://github.com/asgr/ProFound} \citep{Robotham2017,Robotham2018};\ \ProFit: \url{https://github.com/ICRAR/ProFit}
%\citep{Robotham2018};\ \SExtractor: SourceExtractor:
%\url{https://www.astromatic.net/software/sextractor/} or
%\url{https://sextractor.readthedocs.io/en/latest/} \citep{Bertin1996}. }
%
%\facilities{ Hubble and James Webb Space Telescope Mikulski Archive
%\url{https://archive.stsci.edu}\ }



